Performance study of a $3\times1\times1\mbox{ m}^3$ dual phase liquid Argon Time Projection Chamber exposed to cosmic rays

We report the results of the analyses of the cosmic ray data collected with a 4 tonne (3$\times$1$\times$1~m$^3$) active mass (volume) Liquid Argon Time-Projection Chamber (TPC) operated in a dual-phase mode. We present a detailed study of the TPC's response, its main detector parameters and performance. The results are important for the understanding and further developments of the dual-phase technology, thanks to the verification of key aspects, such as the extraction of electrons from liquid to gas and their amplification through the entire one square metre readout plain, gain stability, purity and charge sharing between readout views.

==> Sections/_old/Characteristics.tex <==
%2 parts long run and field scans 
\subsection{Experimental setup}
The \three detector is described in detail in \cite{Aimard:2018yxp}. It consists of a \three liquid argon volume instrumented with a cathode at the bottom and surrounded by a field cage. A charge amplification and anode readout stage is positioned in the gas phase a few millimetres above the liquid argon surface. 
A view of the  detector geometry with  around 30 reconstructed cosmic muon track candidates is presented in \figref{fig:311-geometry}. A zoom around the signal amplification region is also shown. In \tabref{tab:lar-prop} some of the relevant detector features for this paper are listed.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/Characteristics/311-geo-2.png}
\caption{The \three geometry with about 30 reconstructed cosmic muon tracks. Only reconstructed hits from view 1 are shown and the color scale represents the acquired hit charge integral in fC.}
\label{fig:311-geometry}
\end{center}
\end{figure}
At the passage of an ionising particle inside the liquid, electron ion pairs are created. They are drifted towards the surface at a velocity of about 1.6 mm/$\mu s$ thanks to the nominal electric field of 500 V/cm provided by the cathode and drift cage system. Scintillation photons with wavelength peaked at 128 nm are also produced and detected by an array of five PMTs placed at the bottom of the cryostat. They provide the trigger and the reference time for the event with an accuracy of a few nanoseconds. The produced charge is free to drift in the ultra pure liquid argon up to the the surface where it is extracted to the gas phase with a near 100\% efficiency. Once in the gas the drifting electrons are multiplied by Large Electron Multipliers (LEMs) and collected on a two-dimensional and finely segmented anode. The amplification in the LEMs allows to produce signals with amplitudes which are significantly above the level of the ambient noise, resulting in a high quality and good resolution image of the interacting particles. The electron extraction, amplification, and collection are performed inside a \SI[product-units=power]{3x1}{\meter} frame called charge readout plane (CRP). The CRP is electrically and mechanically independent from the drift cage and can be remotely adjusted to the liquid level. The electrons are efficiently extracted from the liquid to the vapour by applying an electric field in the liquid above \SI{2}{\kilo\volt/\cm} \cite{Gushchin:1982}. This electric field is provided by a \SI{3}{\mm} pitch extraction grid positioned \SI{5}{mm} below the liquid argon surface. Once amplified inside the LEM holes, the charge is collected on a two-dimensional segmented anode which consists of a set of independent strips that provide the $x$ and $y$ coordinates of an event with a \SI{\sim3}{\mm} pitch. The LEMs and anodes have been developed towards unit sizes of \fifty. They are precisely assembled side by side to cover the \SI[product-units=power]{3x1}{\meter} area. The anodes are electrically bridged together so as to provide two orthogonal sets of three and one metre long readout strips called \textit{views}. The anodes are carefully designed in such a way that the amplified charge is equally shared and collected on both views \cite{Cantini:2013yba}. View 0 (view 1) consists of 320 three meter-long (960 one meter-long) strips running parallel to the \textit{x} (\textit{y}) coordinate axis. As example we show in \figref{fig:311-hadr-event} a typical event recorded with the \three, in this case a cosmic ray induced hadronic shower candidate. 
\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/Characteristics/Event-shower-1.png}
\caption{2D event display of a cosmic induced hadronic shower candidate with zooms around the interaction region. The event is shown without the application of any noise filtering algorithms.}
\label{fig:311-hadr-event}
\end{center}
\end{figure}
For each view the charge recorded per channel number as a function of the drift time are plotted and the color scale is proportional to the amplitude of the signal. The readout pitch on the horizontal axis is 3.125 mm and the drift time acquisition window of 667 $\mu$s is digitally sampled at 2.5 MHz which results in 1667  time samples. At 500 V/cm drift field this results in a $\sim$0.64 mm spatial resolution of the event along the drift coordinate. The TPC therefore provides a high resolution digitised image of the interaction products with pixel unit sizes of $\sim$ 3.125*0.64 mm$^2$. The contrast of the image (the color scale) is directly proportional to the amount of charge collected on the strips and needs to be maximised for efficient track reconstruction and particle identification. A list of relevant parameters of the TPC charge readout section along with properties of the liquid and gas argon are provided in \tabref{tab:lar-prop}.

\begin{table}[h!]
\renewcommand{\arraystretch}{1.2}
\begin{center}
%\begin{tabular}[\textwidth]{lll}
\begin{tabular}{p{.65\textwidth}p{.2\textwidth}p{.1\textwidth}}
  \toprule
  property & value & unit \\
  \midrule
  \textbf{TPC charge readout} & &\\
   active area   & 3 $\times$ 1 & m\\
    N LEMs (anodes) & 12 & \\
    readout strip width &3.125 &mm\\
    readout strip length View 0 (View 1) & 3 (1)&m\\
    number of channels View 0 (View 1) & 360 (960)&\\
    drift length (time) &1 (607)&m ($\mu$s)\\ 
    drift time digital sample & 400 & ns\\
    drift time acquisition window & 667 & $\mu s$\\
    N drift time digital samples & 1667&\\
    N Pixels $N_{channel}^{charge} \times N_{sample}^{drift}$ View 0 (View 1)& 0.5 (1.6) & MPixel\\
    
    %preamplifier sensitivity ( T$\sim$100 K, $Q<400$ fC)& 3.75 & mV/fC\\
    %amplitude digital conversion & $\sim$0.5 & mV/ADC\\
    digital integral to charge conversion View-0 (View-1) & 55 (66) & ADC/fC\\
    $\tau_1,\tau_2$ for view-0 (View-1) & 6.9, 0.5 (2.2,0.9) &\SI{}{\micro\second}\\
    \midrule
 \textbf{liquid and gas argon properties} & &\\   
  ionisation energy $W_{ion}$ \cite{PhysRevA.9.1438}& 23.6$^{+0.5}_{-0.5}$ &eV \\
   electron drift velocity at 500 V/cm (1 kV/cm)\cite{Li:2015rqa} & 1.648 (2.261) & mm/$\mu$s \\
   ion drift velocity ($\Ed{drift}<1$ kV/cm)) \cite{lar-prop,palestini}& 8 & mm/s\\
   Average (most probable) energy loss for M.I.P & 2.1 (1.7) & MeV/cm\\
   \Wb for M.I.P  at 500 V/cm (1 kV/cm) & 71 (75)& \%\\
   $\sigma_{T}$ for 1 m drift \cite{Li:2015rqa}& 1.2& mm\\
   $\sigma_{L}$ for 1 m drift \cite{Li:2015rqa} & 0.9& mm\\
   $\mathscr{A}$ 100 ppt (30 ppt) longest drift & 94 (96)&\% \\
   %Charge extraction efficiency at \Ed{extr}=1.5, \Ed{extr}=2 kV/cm \cite{}& 60 (90)& \%\\
    GAr temperature near LEMs during data taking \cite{Aimard:2018yxp} &90$\pm0.5$ & K\\ 
    cryostat pressure during data taking \cite{Aimard:2018yxp} &1000$\pm 1.4$ & mbar\\
    First Townsend coeff. $\alpha$ for \Ed{LEM}= 28, 33 kV/cm& 20.7, 43.1 & cm$^{-1}$ \\
    %First Townsend coeff. $\alpha$ for \Ed{LEM}= 28, 33 kV/cm& 20.7, 43.1 & cm$^{-1}$ \\
   %nuclear interaction length & 84& cm\\
   %radiation length & 14 & cm\\
  \bottomrule
       \end{tabular}
     \end{center}
     \caption{\label{tab:lar-prop} Some parameters relating to the imaging of the TPC along with a summary of coefficient used for the analysis in this paper. Unless otherwise indicated all values are taken from Ref. \cite{NIST:LAR} computed for a liquid with temperature of 87.3 K, pressure of 1 atm and drift electric field $\Ed{drift}=500$ V/cm. }
   \end{table}
\subsection{Effective gain and signal to noise ratio}
An ionising particle depositing an energy $\Delta E_{dep}$ in the liquid produces an ionising charge that is free to drift of $\Delta Q_0=(\Delta E_{dep}/W_{ion}) \cdot \Wb$ where $W_{ion}$ is the ionisation work and \Wb denotes the remaining fraction of produced electrons that don't immediately recombine with the ions. The latter depends on the ionisation density and the drift field and is well parameterised by Birk's Law \cite{tagkey1964iii}. The values $W_{ion}$ and \Wb are reported in \tabref{tab:lar-prop}. At a drift electric field, \Ed{drift} of 500 V/cm a minimal ionising particle (M.I.P) produces a charge yield $\Delta Q_0$ of about 1 fC/mm.
The charges drift for a duration $t_{drift}$ and electron attachment to impurities in the liquid attenuates the signal by a factor $A=e^{-t_{drift}/\tau_e}$ where $\tau_e$ is called the electron lifetime. Its value is dependent on the performance of the cryogenic purification and recirculation system. As shown in \cite{Aimard:2018yxp} preliminary study of the data suggest a $\tau_e \approx 5 $ ms or an oxygen equivalent\footnote{$\tau_e[\mbox{ms}]\approx$300/\oxeq [ppt]} impurity level of $\sim$60 ppt \oxeq.

The amount of charge deposited by a MIP and collected on an anode strip can therefore be written as:
\begin{equation}\label{eq:dq}
 \Delta Q_{anode}^{mip} \approx \Delta Q_{0}^{mip} \cdot \mathscr{A}(\tau_e) \cdot \Geff \cdot \frac{1}{2},
\end{equation}
where we neglect the effect of transverse and longitudinal diffusion ($\sigma_{T}$,$\sigma_{L}$) for the relatively short 1 meter drift distance (see \tabref{tab:lar-prop}).
The factor 1/2 represents the fact that the charge yield is equally splitted between both collection views of the anode.  The projected charge on one anode strip, $\Delta Q_{anode}^{mip}$, depends on the azimuthal and polar angles of the track crossing the TPC fiducial volume. It will be minimal for horizontal tracks ($\theta=90^\circ$, as defined in \figref{fig:311-geometry}) and larger for vertical tracks ($\theta=180^\circ$). The impact of the track angles on the signal is discussed in more detail in \secref{sec_det-response}. 

\Geff~is the \textit{effective gain} of the dual phase chamber which primarily relies on the multiplication factor of the electrons inside the LEM holes but also depends on the overall electron transparency (${\cal T}\leq1$) of the extraction grid, LEM and anode inside the CRP. The effective gain can be analytically decomposed as:
\begin{eqnarray}\label{eq:gain_func}
\Geff&=&{\cal T}\cdot \GLEM\\
\GLEM&=& \exp\left[{\alpha\cdot x}\right]\\
\alpha&=&A\rho \cdot \exp\left[{-B \rho/\Ed{LEM}}\right],
\end{eqnarray}
where $\alpha$ is the first Townsend ionisation coefficient for an amplification field \Ed{LEM} inside the LEM hole and gas density $\rho$; $x$ denotes the effective amplification length. $A$ and $B$ are parameters which depend on the gas properties and are obtained from numerical calculations \cite{magboltz}. Their values along with the nominal pressure and temperature of the gas argon during operation of the detector are reported in \tabref{tab:lar-prop}. Stable effective gains of around 20 
have been reported inside liter-scale dual phase TPCs \cite{Cantini:2013yba,Cantini:2014xza} by operating the CRP at the electric field settings shown in \figref{fig:311-geometry}. First analyses of a data subset collected in the \three suggests a $\Geff\approx3$. The \three is limited in effective gain due to the high voltage issues on the grid and LEM reported in \cite{Aimard:2018yxp}.

The value of \Geff directly impacts the imaging quality of the event and is hence used as a fundamental  quantity  to  benchmark the detector performance. 
Most importantly it drives the signal to noise ratio of the TPC ($S/N$) which is defined as the ionisation charge collected on one anode strip divided by the Equivalent Noise Charge (ENC) of the strip:

\begin{equation}
    S/N=\frac{\Delta Q_{anode}^{mip} \mbox{[fC]}}{\mbox{ENC [fC]}}\equiv\frac{\mbox{ionisation charge collected on one anode strip}}{\mbox{ENC RMS}},
\end{equation}

where $\Delta Q_{anode}^{mip}$ is defined in \equref{eq:dq}. The ENC on a channel is the combination of the intrinsic noise due to the input capacitance of the anode strips and all other sources of coherent or incoherent noise which may by picked up. First measurements \cite{Aimard:2018yxp} suggest and ENC of below $\sim$2000 electrons (0.32 fC) for both views when the TPC is operating. A more detailed analysis of the noise during data taking has been performed and is discussed in \secref{sec_noise}. \figref{fig:gain-var}-right illustrates the expected $S/N$ for a MIP crossing the detector horizontally as a function of \Geff and drift distance for a LAr purity of 50 ppt [O$_{2}]_{\mbox{eq}}$ and 500 V/cm drift field. 
\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/Characteristics/number_electrons_MIP_drift_and_gain}
\caption{Left: relative fluctuation of \GLEM around its nominal value a when varying the gas density and LEM thickness. The fluctuation is shown for two different values of \Ed{LEM}. Right: number of ionisation electrons from a MIP interaction collected per view on one anode strip as a function of the effective gain and drift distance.}
\label{fig:gain-var}
\end{center}
\end{figure}
The value of 50 ppt is approximately the one that has been achieved for long duration in the \three as already shown in \cite{Aimard:2018yxp} and detailed in \secref{sec_e_lifetime}. For the rather modest one meter drift of the \three a $S/N$ of near 10 can be expected even at an effective gain of around 1-2. The importance of the effective gain becomes clear with increasing drift distances. Operating with $\Geff\approx10$ would correspond to obtaining $S/N$=100 for one meter drift and around 10 for 12 meter drift. Twelve meters is the drift distance of the proposed DUNE 10kt dual phase detector \cite{DUNE_CDR}. The plot illustrates the importance of the effective gain especially if the targets in terms of noise performance or LAr purity are not met.

In order to have a uniform and stable effective gain, the electric field across the LEM, its thickness as well as the density of the argon vapour must all be carefully controlled. This is illustrated in \figref{fig:gain-var}-right: due to the exponential nature of \Geff, variations in the \fifty LEM thickness or fluctuations in the gas density may have a relatively large impact on its value. In the \three the thickness uniformity of all the \fifty LEM plates was carefully checked and the gas argon density was maintained at a stable value. Both were uniform within typically one percent (see Ref. \cite{Aimard:2018yxp} and \tabref{tab:lar-prop}), which would translate to about $\pm$10 (20) \% on \Geff~ if the LEM is operated at 28 kV/cm (33 kV/cm) and assuming a transparency of one. The obtained uniformity of the effective gain in the \three is discussed in \secref{sec_uniformity}.

%\subsubsection{Charge extraction and electrical transparency}
At a given LEM amplification field, the electrical transparency $T$ is essentially driven by the values of the extraction and induction fields. Both are discussed below. TODO.

%As discussed in \cite{Aimard:2018yxp}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/Characteristics/Extr_slow_fast.png}
\caption{Left: electron extraction time constant as a function of the extraction field in the liquid. Right: extraction efficiency for the fast and slow component as a function of the electric field in the liquid. The data points are taken from \cite{}.}
\label{fig:gain-var}
\end{center}
\end{figure}


 
\subsection{Charge readout detector response}


TODO: Describe the MC simulation done in flat space to characterise the readout, response for different angles with the preamplifier response included

% This is the case for near vertical tracks where the time extension of the drifting electron cloud on a given strip is in the tens or hundreds of micro-second range.

% Current pulses of more than 1 us will occure 
% where the time over which the electrons are extracted reduces, will introduce larger tails in the waveform. The impact is discussed in more detail in \secref{sec:waveform-simu}.

% This is typically the situation at occurs at low extraction efficiency. Above 2 kV/cm of extraction in the liquid all the charge is extracted with a time constant
% This effect Where for an equal amount of collected electrons the waveform tends to flatten out with 
% This is the case for near vertical tracks where the time extension of electron cloud on a given strip is in the tens or hundreds of micro-second range. This is illustrated in \figref{fig:waveform-high-theta}, showing the average waveform for reconstructed tracks at different $\theta$ angles.
% The shape of the waveform in terms of amplitude, width and integral is an important parameters that shape the imaging quality of the detector. The response of the detector to will thus depend on the duration of the pulse and thus on quantities such as the track inclination, the electron extraction time constant,... For an equivalent amount of charge some hits may be more delicate to reconstruct because of their topology.


% where pulses of long duration were injected.

% The waveform integral is also affected as illustrated in \figref{fig:pulse-comparison-views}-right. 
% since the boards feature a 2 nF DC decoupling capacitor at their input 
% The difference of the waveform shapes between both views arises from the the preamplifier decouping stage being connected to an capacitive load and their difference capacitive loads. Constant ratio of about 20\% which accounts for the different calibration constants needed to convert the digitised integral values into fC are retreived by injecting charge in the 0-160 fC range and fitting with a liear fit. This is

% The conversion
% Their difference in amplitude

% By pulsing over an extented range Linear fits
% mainly because of the differences in capacitive loads from the one meter on one hand and 3 meter strips.
% As understood from \equref{eq:gain_func},

% The values of $\tau_1$ and $\tau_2$
% Due to the differences in input capacitances from the strip length
% From the convolution one understands that if the duration of the current pulse is of the order of the peaking time of the response function peaking time , for longer durations however the convolution provides longer pulses with smaller amplitudes  For injected current pulses of short  duration of typically less than \SI{1}{\micro\second}

% The by a charge injection system present at the extremities of the readout strips.

%We already showed that the response function repredocues well the the 






%\subsection{Evolution/Stability of LAr purity and GAr density during data taking period}
%\subsection{Study of the noise and its evolution over the data taking period}

%according the arrival time of the electron elecron cloud of


%The electron cloud diffusion is thus expected to have a negligible impact on the amount of collected charge or the response of the preamplifier.


 
%Depending on the arrival position of the drift charge on the anode strips currents are induced on the corresponding readout electrodes of the di↵erent views.

%The charge The output digitised signal is performed by parametrisating the waveform from the data

%is also simulated with an electron lifetime defined by of 5 ms, which is the average value found results in almost neglible values well as transverse and longitudinal diffusion
%which includes the digitisation following an accurate description of the preamplifier response. 

%Non-uniformities in the electric field may induce distortions of the projected in order to check for possible and it is therefore important to accureately simulate the drift field. 


%\subsection{Detector simulation}

% \subsection{Description of the detector simulation and generated MC sample}
% Show a fitted waveform and compare: 3 m vs 1m, low and high extraction field, (low and high induction field?), low and high amplification, (low and high drift?)
% show that we can fit it properly

% \subsubsection{Electric fields along the drift}
% drift velocity in liquid, in gas, focusing of the grid
% Extraction field. Effect of non planarity of DC and CRP on the field.
% \subsubsection{Transverse and longitudinal diffusion}
% In the liquid (in the gas?)
% %\subsection{Extraction field}



==> Sections/_old/Performance-Analysis.tex <==


% Another important parameter that shapes the response of the detector is the time duration of the current pulse.  shown in \cite{Aimard:2018yxp} and as also understood from  if the duration of the input current pulse becomes larger than the $\sim$\SI{1}{\micro\second} peaking time of the response function the waveform will reduce in amplitude and extend in width. As expected the value of the integral, which only depends on the amount of charge is conserved. This is verified in \figref{fig:pulse-comparison-views}-right. 
% For an equal amount of charge deposited on the anode strips, the amplitude of the signal thus depends on the duration of the current pulse. Parameters such as the track inclination but also extraction field will thus have an impact on the signal amplitude.
% At low extraction electric fields in the liquid (typically below..) the extraction time constant of one micro second the extraction field where a fraction of the electrons is extracted with time constants in the us range. The impact of track topology and extraction eff is discussed in more detail in \secref{sec:waveform-simu}. 

% \begin{figure}[h!]
% \centering
%  \includegraphics[width=.7\textwidth]{Figures/DetResponse/Waveform_extr.pdf}
%  \caption{Waveform from similar cosmic muon tracks at different extraction fields.}
%  \label{fig:waveform_extr} 
% \end{figure}




% tracks have the expected 3 fC from a MIP on one strip.
% due to the projection seen by a strip is if longer time duration projected onto a strip view hmore charge gets collected but over a longer duration resulting in wider hits with more charge.
% larger integrals andAs tracks are more incline and more parrallel to one view illustrating that down-going reconstructed on view 0 The width of the waveform 
% This way the shape of the waveform depending on the track inclination is accurately reproduced in the simulation.

% Meaning that for both data an
% In order to accurately reproduce as much as possible the data the distortions of the waveforms coming from low extraction fields are included based on paramtration from the data.

% which accounts for 
% The response function is applied to 
% The main parameters which distort the waveform are the extraction field the noise both are taken from the data.

% that are included in the simulation

\subsection{Muon track selection}
As mentioned in \secref{sec_intro} a coincidence of 5 PMTs is used as a decision to acquire the event; this trigger then naturally selects interactions which produce large quantities of light such as muons which cross the entire detector or particles which develop into showers. As discussed in \secref{sec:trigger_simu}, we know from the detector simulation and visual scans that the event sample is near 50:50 divided between showers and muons. One some occasions an event will be composed of both muons and showers. Through going muon tracks are MIPs which deposit a known $<dE/dx> \simeq$2.1 MeV/cm in LAr and are therefore used to characterise the performance of the TPC in terms of effective gain. We have developed two methods to separate muons from showers, one based on cuts and another using a three-hidden-layer multilayer perceptron neural network. Both give similar performance the latter has the advantage that it could be also be used to separate electromagnetic from hadronic showers.
They are briefly described  in the next two subsections.
\subsubsection{Cut based}
As explained in \secref{sec:track_reco} showers will most of the time be reconstructed as many independents clusters which are subsequently fitted  with a straight line producing multiple short "tracks". A selection based on the length of the reconstructed track thus already allows to discard a large fraction of the showers. Only  tracks which have more  than  50 cm are retained. As a reminder, the distribution of the reconstructed track lengths are shown for both MC and data in \figref{fig:tracklength}, where  we clearly see  that most showers have lengths in the 10 cm range. To further clean the sample a second cut based on the output of a dedicated algorithm 
is used. The algorithm scans the hits belonging to a reconstructed track and computes the ratio of the charge contained inside two rectangles positioned according to the reconstructed 3D path of the track as shown in \figref{fig:highway_event}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/Chap4/highway_event.png}
\caption{Illustration of the algorithm  which computes the charge box ratio  on and a muon candiate and EM shower event }
\label{fig:highway_event}
\end{center}
\end{figure}

The ratio of the charge contained in the smaller rectangle to that of the larger one defines a metric called the charge box ratio (CBR) which is assigned to the track. Tracks belonging to showers where the charge is spatially spread out will have large CBR, on the other hand tracks produced by muons will tend to lower CBR values (see \figref{fig:track-sel-cut}-left). An upper limit of 20\% on the CBR is assigned to tag the cluster as a track. This value is based on detailed eye-scans and verified with the Monte Carlo simulation in order to maximise the track selection efficiency and the muon sample purity. 
The breakdown of the the track length and CBR cuts is illustrated in \figref{fig:track-sel-cut}-right. Initially only 5.7\% of all tracks are from muons; after both cuts this number drops to about 4\% with a x\% contamination from showers, corresponding to an efficiency of 70\% and a purity of x\%.
%a relatively pure sample of muons is selected from and  in our final sample 

%in \figref{fig:track-sel-cut}, we show the distribution of the CBR in our Monte Carlo sample for the different categories of particles. 
%as well and the purity of the track sample after both cuts have been applied.
%As can bee  seen from an initial sample
%purity after both set of cuts applied to the sampe. 
%The muon selection efficiency based on this method is  presented in \figref{fig:track_selection_purity}.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/Chap4/CBR-efficiency.png}
\caption{**TMP** Left: distribution of the CBR for all reconstructed tracks in data and MC. Right: effect of the tracj length and CBR cuts on the track selection efficiency.}
\label{fig:track-sel-cut}
\end{center}
\end{figure}

\subsubsection{Multi-variate classification}

An alternative 1selection, based on multivariate classifiers, has been also developed, to use more correlations between variables.Both a Boosted Decision Tree (BDT) and a Multi-Layer Perceptron approach have been studied, with the latter giving slightly better performance, and therefore described here. Three networks were developed, one treating a particle species (muons, pions or electrons) as signal and the others as background. They were trained on a Monte Carlo dataset consisting of 600 events of each of the three species. 
Eight variables were used in the classifier:
\begin{itemize}
    \item $L_{straigth}$ track length along a straight line, distance between start and end point of a track
    \item $L_{trajectory}$ track length trajectory, summing all steps along the trajectory points
    \item $\Delta L/L= \frac{L_{straight}-L_{trajectory}}{L_{straigth}}$
    \item $Q$, amount of charge deposited by a track
    \item $Q/L$, charge divided by track length
    \item number of hits
    \item number of hits divided by track length
    \iten Charge Box Ratio, as defined above
\end{itemize}

The neural network consisted in an input layer with eight nodes, an inner layer with seven, and a single output layer. The distribution of its output variable, in the case when muons are considered as signal and the sum of electrons and pions as background, is shown in figure \ref{fig:nnoutput}. A nice separation between the two classes is observed. The value of the cut on the output variable needed to obtain an efficiency of 70\% on muons, the same as the cut-based analysis, is obtained. The purity, assuming an initial composition of a ratio 1:5:5 for muons, electrons and pions, is 84\%, compared to 62\% of the cut-based method for the same efficiency.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=\textwidth]{Figures/Chap4/nnoutput.jpg}
\caption{Distribution of the output variable of the multi-layer perceptron, when muons are considered as signal, and electrons plus pions as background.}
\label{fig:nnoutput}
\end{center}
\end{figure}


% \subsection{Reconstruction and Hit Finding Efficiency}
% **TBD**
% Now that we have shown that the MC reproduces the data we can check the effect of gain and extraction field on the signal an extrapolate the efficiency for all track topologies and in any given range of field settings.
% \begin{figure}[h!]
% \begin{center}
% \includegraphics[width=\textwidth]{Figures/Chap4/gain_map.png}
% \caption{gain map. ** show S/N instead of signal amplitude**, also show the reconstruction eff with different lifetimes?}
% \label{fig:gain-map}
% \end{center}
% \end{figure}

% We therefore define the S/N ratio as a fundamental parameter which characterises the TPC performance.

% The S/N defined in sec is therefore an esential parameter. The more electrons the higher the amplitude. 

% This S/N is essentially driven by the effective gain of the TPC

% Evidently the efficiency for identifying the hits above the ambient noise is driven by the amplitude of the peak which is primarily driven by the amount of charge reaching the amplifiers. The shape of the signal is dicussed in more detail in \secref{sec_det-response}.





% \begin{figure}[h!]
% \begin{center}
% \includegraphics[width=\textwidth]{Figures/Characteristics/dqds-data-mc}
% \caption{\dqds data and Monte Carlo}
% \label{fig:noise-removal-waveform}
% \end{center}
% \end{figure}

% \begin{figure}[h!]
% \begin{center}
% \includegraphics[width=16cm]{Figures/Chap4/track2d.png}
% \caption{}
% \label{fig:track-selection}
% \end{center}
% \end{figure}






%this is discussed in more detail in  the next \secref{sec_det-response}.

%The procedure is validated by Monte Carlo (see 

% Since for the characterisation of the TPC are only interested in selecting a high purity of muoj samples,  shower like events are discarded by offline tools described 
% and shower like events are separated from muons at a later stage during the offline analysis with procedure described in \secref{sec:}.



%  This reconstruction process allows to reconstruct downward going muon tracks with an efficiency of $\sim$98\% (see \secref{sec:rec_eff}). This process is applied to all event topologies. Shower like events, such as hadronic or electromagnetic showers in \figref{fig:mc_data_events} or hadronic showers and seperation between muon track and shower candidated is performed offline and described in \secref{sec:}.



 
%Once the two-dimensional clusters are formed, the final step of reconstruction consists of
%matching the energy deposit between the two views to build a tri-dimensional representation
%of the event.

%The clustering kinks
%Efficient hit finding on both views constitutes the fundamental prerequisite 
%which requires a good signal to noise ratio on both views before any noise subtraction is applied. Is therefore driven by the ease withc wich we can identify peaks even even before the application of noise algo.


==> Sections/_old/Plans.tex <==

Relevant physical parameters to describe the detector.
what may affect the detector response?
What impacts the performance of the detector?

uniformity of density (effect of pressure and temperature), liquid level fluctuation (are they important), change of v drift between gas and liquid, bent tracks, electric field
Grid focusing, electric fields, LEM dead area

1. Compare true and reconstructed data (Nb of track, geometry, charge)
2. Study the effect of diffusion, noise, slow extraction, ...
3. Understand the data we have muon flux vs PMT trigger/CRT trigger, ...
4. Which method is "correct" for dQ/ds (MPV, tr. mean, median, log-norm fit, ...)

We need Mc to validate dQ/dx, purity
function 
MC-> effect of slow drift
effect of gain on reconstruction effeincy
somedy effect of LEM-amp on reconstruction effiency 
1. Start with flat phase MC (because its there) and produce ROOT files (Christoph)
2. produce realistic MC track sample, biased track topology and real cosmic flux (Khai with help Jose)
3. include realistic noise in MC (Christoph)

4. include gas field map? Laura MB

5. Study hit and track reconstruction efficiency on straight tracks
effect of slow extraction on rec eff
effect of low induction on rec eff
effect of diffusion (longitudinal and transverse)
effect lifetime on rec-eff
effect of dead areas on hit reco
effect of dx on MPV (mean if any?)

6.Compare MC and data
 comparison of theta, phi and basic geometrical parameter
 compare gain uniformity and dead areas (map the data uniformity in the MC?)
 compare data/MC waveforms
 compare data/MC dQ/dx

7. Organisation: organise root files (CERNbox, ..) have official root files, official version official cuts (Lauras+ Sebastien) 1 week
CERN-box data and MC official naming for files 

-----------------------
3. Detector response and simulation
3.1 Definition of effective gain and parameters that may affect the dual phase TPC
(CRP bending, pressure temperature)
3.2 Description of the detector simulation and generated MC sample
3.4 Charge readout detector response (injected pulse)
3.5 simulation of the dual phase detector response
(slow extraction, diffusion, extraction grid, bunching)
3.3 Reconstruction procedure 

4. hit and track reconstruction efficiency and effect of DP parameters
%how me measure effective gain in the TPC ( dQ/ds definition),...


%uniformity of densitigrid

% \subsection{Collected data}
% \subsection{charge sensitive preamplifier response and calibration}
% \subsection{Detector simulation}
% Gain, extraction and induction efficiency implementation
% Noise filtering test

% \subsection{Reconstruction of cosmic events}
% -Recap of the different coordinates used (CRT, light, DAQ, softwares)
% -Robustness of the reconstruction in terms of track parameters
% -3m Vs 1m view , charge asymmetry 
% -Define a common reconstruction version which everybody uses
% -Performance of noise filtering
% -Hit finding efficiency
% -Geometrical reconstruction ? (ie different hit finding parameters for views and possibly channels)
% -Pressure, temperature and liquid argon stability and possible corrections (if needed)

% \subsubsection{straight tracks}
% \subsubsection{Hadronic interactions}
